Efficient All-to-All Collective Communication Schedules for Direct-Connect Topologies

The all-to-all collective communications primitive is widely used in machine learning (ML) and high performance computing (HPC) workloads, and optimizing its performance is of interest to both ML and HPC communities. All-to-all is a particularly challenging workload that can severely strain the underlying interconnect bandwidth at scale. This paper takes a holistic approach to optimize the performance of all-to-all collective communications on supercomputer-scale direct-connect interconnects. We address several algorithmic and practical challenges in developing efficient and bandwidth-optimal all-to-all schedules for any topology and lowering the schedules to various runtimes and interconnect technologies. We also propose a novel topology that delivers near-optimal all-to-all performance.

==> concl.tex <==
\vspace{-2ex}
\section{Conclusion}\label{sec:conclusion}
We develop efficient schedules and topologies for alltoall collective communications geared for large-scale direct-connect supercomputer interconnects.
Algorithmically, we enhance the scalability of the multi-commodity flow (MCF) framework by decomposing and parallelizing the problem. 
We additionally develop a software stack for lowering the optimal MCF solutions to both accelerator and HPC fabrics, with and without extra NIC forwarding bandwidth.
We establish a lower bound for all2all performance, and we propose a novel generalized Kautz topology that has superior alltoall performance and better coverage of the topology space than the state-of-the-art. 


